ViTa-SLAM: A Bio-inspired Visuo-Tactile SLAM for Navigation while Interacting with Aliased Environments

RatSLAM is a rat hippocampus-inspired visual Simultaneous Localization and Mapping (SLAM) framework capable of generating semi-metric topological representations of indoor and outdoor environments. Whisker-RatSLAM is a 6D extension of the RatSLAM and primarily focuses on object recognition by generating point clouds of objects based on whisking information. This paper introduces a novel extension to both former works that is referred to as ViTa-SLAM that harnesses both vision and tactile information for performing SLAM. This not only allows the robot to perform natural interaction with the environment whilst navigating, as is normally seen in nature, but also provides a mechanism to fuse non-unique tactile and unique visual data. Compared to the former works, our approach can handle ambiguous scenes in which one sensor alone is not capable of identifying false-positive loop-closures.

==> Makefile <==
# Makefile to create PDF documents from LaTeX-Files
PROJECT=vita_slam_cbs_19
TEX=pdflatex
BIBTEX=bibtex
PDFVIEWER=evince
PDF=$(PROJECT).pdf
BUILDTEX=$(TEX) $(PROJECT).tex


all:
	$(BUILDTEX)
	$(BIBTEX) $(PROJECT)
	$(BUILDTEX)
	$(BUILDTEX)
	$(MAKE) close-pdf
	$(PDFVIEWER) $(PDF) & echo $$! > $(PDFVIEWER).PID  # Store the process ID of PDF viewer
	$(MAKE) clean

clean-all:
	@rm -f *.dvi *.log *.bak *.aux *.bbl *.blg *.idx *.ps *.eps *.pdf *.toc *.out *~
	echo "Cleaned all binaries"

clean:
	@rm -f *.log *.bak *.aux  *.blg *.idx *.toc *.out *~ *.sta
	echo "Cleaned Binaries"


close-pdf:
	# If old pdf is already open, close it first then open a new one.
	if [ -e $(PDFVIEWER).PID ]; then \
	   	kill -TERM $$(cat $(PDFVIEWER).PID) || true; \
	fi;

.PHONY : all clean

